Effective Label Propagation for Discriminative Semi-Supervised Domain Adaptation

Semi-supervised domain adaptation (SSDA) methods have demonstrated great potential in large-scale image classification tasks when massive labeled data are available in the source domain but very few labeled samples are provided in the target domain. Existing solutions usually focus on feature alignment between the two domains while paying little attention to the discrimination capability of learned representations in the target domain. In this paper, we present a novel and effective method, namely Effective Label Propagation (ELP), to tackle this problem by using effective inter-domain and intra-domain semantic information propagation. For inter-domain propagation, we propose a new cycle discrepancy loss to encourage consistency of semantic information between the two domains. For intra-domain propagation, we propose an effective self-training strategy to mitigate the noises in pseudo-labeled target domain data and improve the feature discriminability in the target domain. As a general method, our ELP can be easily applied to various domain adaptation approaches and can facilitate their feature discrimination in the target domain. Experiments on Office-Home and DomainNet benchmarks show ELP consistently improves the classification accuracy of mainstream SSDA methods by 2%~3%. Additionally, ELP also improves the performance of UDA methods as well (81.5% vs 86.1%), based on UDA experiments on the VisDA-2017 benchmark. Our source code and pre-trained models will be released soon.

==> ECCV20_rebuttal.tex <==
\section{REBUTTAL}

%##########
\subsection{For AC and PC}
Due to the fact that the reviewers come from weakly related research fields or just read similar work, they may not be familiar with the core problems and the experimental settings of domain adaptation, and have made some questionable comments (e.g., Q1 and Q4 of Reviewer2; Q3 and Q5 of Reviewer3). All these comments indicate that they are not familiar with the area and therefore have underestimated the contributions of our work.

We try our best to meet the inquiries and concerns from reviewers and will revise our paper and release our code to make it easier to follow.

%########## reviewer 1 [read similar work] [有希望]
\subsection{REVIEWER $\#1$}
We thank the reviewer for the positive feedback and constructive suggestions on our paper. We hope the answer satisfactory and we will revise the paper to make it easier to follow.

Q1) The motivation for the CDL is somewhat unsatisfactory. \\
A1) % @ 200527
%Most DA methods try to learn a feature extractor for domain alignment, but for the complicated DA problem, this is still not perfect enough. Besides aligning feature in the domain level, we proposed a method (CDL) to align feature in the class level.
% @ 200528
(i) Most DA methods align the features in a domain-aware manner, which ignore the discrimination of features in the class level. To this issue, we propose the CDL to facilitate the consistency of the semantic (class-aware) information between the two domains.
(ii) The $\cdl$ can be re-written:
\begin{equation*}
\begin{split}
    \cdl &= - \frac{1}{| B^{\Sdomain} |} \sum_{X_{i}^{\Sdomain} \in B^{\Sdomain}}{\yyp\log(\yym)} \\
    & ( \lim_{ \yyp \to 0+ } \yyp \log( \yyp ) = 0, \quad  \lim_{ \yyp \to 1 } \yyp \log( \yyp ) = 0) \\
    &= \frac{1}{| B^{\Sdomain} |} \sum_{X_{i}^{\Sdomain} \in B^{\Sdomain}}[ \yyp\log(\yyp) - \yyp\log(\yym)] \\
    &= \frac{1}{| B^{\Sdomain} |} \sum_{X_{i}^{\Sdomain} \in B^{\Sdomain}}{ \yyp \log( \frac{\yyp}{\yym} ) }
\end{split}
\end{equation*}
That is, to minimize $\cdl$ is equal to minimize the KL-divergence from $\yym$ to $\yyp$.
$\yyp$ is the probability distribution based on cycle consistency or mutual nearest neighbors, %$\cdots$ [+ ASSUMPTION + What the interpolation in (2) implies in the target domain],
and $\yym$ is the probability distribution based on the learned features.
Thus, the objective of $\cdl$ is to propagate information from $\yyp$ to $\yym$, to learn to model $\yyp$ with $\yym$, and to make $\yym$ discriminative.

Q2) The novelty on using mixup seems somewhat incremental. \\
% @ 200525
% A2) (i) The novelty on using mixup is only a part of the proposed method. The major novelty is that a novel and effective cycle consistency loss $\cdl$ for inter-domain propagation and an effective self-training strategy to improve the label consistency in the target domain. (ii) Small as it is, building on the results in Table.5, the change proves to be quite effective. (iii) During our experiments, we attempted to propose other mixup strategies, but failed to achieve better performance.
% @ 200526
A2) (i) The balanced mixup is a simple and effective improvement over the original mixup. It outperforms the original version by $1.5\%$, see Table.5. (ii) The proposed ELPNet consists of two novel components: a new cycle discrepancy loss and a new intra-domain label propagation scheme.

Q3) The fixed interpolation might incur some ill effects. \\
A3) %(i) In the vanilla supervised learning problem where the ground truth labels are given, the fixed interpolation can incur negative effects. On the other hand, in the self-training stage of one domain adaptation method where no manual annotation is available, the fixed strategy of mixup helps $\cdots$ (ii) After reading [1] below, we admit that the balanced mixup might suffer from manifold intrusion issue, which is an interesting question and beyond the scope of this paper.
% @ 200528
The discussion about manifold intrusion in [1] above is interesting. Admittedly, balanced mixup might incur some unknown negative effects. On the other hand, at least in this paper, the proposed balanced mixup provides $1.5\%$ gain over the original mixup, and how to deal with manifold intrusion is not the core problem and beyond the scope of this paper. 

%Q4) For a future revision of the paper or future work, I would find it interesting to study the effect of more advanced mixup strategies. \\
%A4) It is a good and interesting question.

%########### reviewer 2 [published weakly related work] [补充 method detail 的同时，再次强调结果；会公开代码，便于理解]
\subsection{REVIEWER $\#2$}
We thank the reviewer for the positive feedback. We will explain your concerns point by point. We will revise the paper to make it easier to follow and release the code to elaborate the implementations.

Q1) Are there any reasons why different CNN architectures were used for different datasets? \\
A1) (i) For fair comparisons, we use the same backbone as the baselines applied. 
(ii) The effectiveness is more convincing, if one method consistently performs better on various backbones.

Q2) The proposed method has been trained on ImageNet but is evaluated on smaller target domains. \\
A2) In domain adaptation, (i) pre-training on ImageNet before training on the source domain (not ImageNet) is a common practice and the baselines compared in this paper are all pre-trained on ImageNet; (ii) for reliable comparisons, the evaluations are based on the average results of different settings, where various scale domains are selected as the source domain.

Q3) It is not clear how the authors find the correct projection across different domains. %I believe the quality of the paper could be improved with further descriptions about their cross domains projection method.
\\
A3) To find the effective projection across domains, we conduct inter-domain propagation using the proposed CDL, which exploits the cycle consistency. Besides, we use intra-domain propagation to benefit the discrimination of learned features in the target domain, and further refine the correct projection from source domain to target domain, which is the goal of domain adaptation.

Q4) How did you set these hyper-parameters? \\
A4) We set the hyper-parameter via cross-validation experiments.

%########### reviewer 3 [published weakly related work] [结果好，但不清楚为何 | 熟悉 TCC，argue 与 MME 的对比不合适]
\subsection{REVIEWER $\#3$}
We thank the reviewer for the positive feedback and constructive suggestions on our paper. We will revise our paper to introduce missing details and make the paper easier to follow.

Q1) For the UDA results on VisDA-2017, how do you train the ELPNet? \\
A1) (i) We train the ELPNet by following the common practice of UDA. The proposed ELPNet still works without labeled target data. (ii) As described in line 494, we conduct ELPNet on the framework of DTA [14]. Specifically, we utilize CDL and our self-training strategy to improve performance. We will release the code to elaborate the experiment details. % The authors should further elaborate on the difference with the SSDA experiment setting.

Q2) The authors should clarify why aligned features alone do not guarantee good performance. %Could the proposed method guarantee good enough results?
\\
A2) (i) As pointed in [20], the methods that are good at feature alignment might enhance the transferability of representations at the cost of discriminability. We wanted to express the same idea but used some confusing words. (ii) We are sorry for the unnecessary controversy, and we will revise the paragraph to make it more objective and reasonable.
%承认措辞有些问题; 再做解释; 事后会进行修正。

Q3) It is unclear to me why the proposed CDL can improve DA performance. \\
A3) (i) Inspired by TCC [28] that aligns each videos via cycle consistency, we propose the CDL to exploit cycle consistency and facilitate feature alignment between the source domain and the target domain in a semantic-aware manner. (ii) Please also refer to A1 of Reviewer$\#1$.

Q4) %The previous SSDA [7] conducted the experiments with different networks, while
The authors only report the performance in one backbone. \\
A4) We conduct additional experiments on VGG-16 and our method still outperforms other SSDA methods. Due to the limited time, we randomly select $4$ adaptation settings from DomainNet. We hope these results (including the table in A4) can satisfy this question.
\begin{table}[h]
    \centering
    \caption{Results ($\%$) on DomainNet benchmark using VGG-16 and ResNet-34.}
    \label{tab:DomainNet_withVGG16}
    \setlength{\tabcolsep}{1.8mm}{
    \begin{tabular}{l|cccccccc|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{R to C} & \multicolumn{2}{c}{P to C} & \multicolumn{2}{c}{S to P} & \multicolumn{2}{c|}{P to R} & \multicolumn{2}{c}{MEAN} \\
            & \footnotesize{1shot} & \footnotesize{3shot} & \footnotesize{1shot} & \footnotesize{3shot} & \footnotesize{1shot} & \footnotesize{3shot} & \footnotesize{1shot} & \footnotesize{3shot} & \footnotesize{1shot} & \footnotesize{3shot} \\
        \hline
        \multicolumn{11}{c}{VGG-16 (NEW)} \\
        \hline
        MME & 60.6 & 64.1  & 57.0 & 60.7 & 60.5 & 60.9 & 72.2 & 75.3 & 62.6 & 65.3 \\
        Ours & 62.5 & 65.5 & 59.2 & 63.0 & 72.8 & 62.1 &  & 76.0 &  & 66.7\\
        \hline
        \multicolumn{11}{c}{ResNet-34} \\
        \hline
        MME & 70.0 & 72.2 & 69.0 & 71.7 & 64.8 & 66.8 & 76.1 & 78.5 & 70.0 & 72.3 \\
        Ours & 72.8 & 74.9 & 72.0 & 74.4 & 66.7 & 69.7 & 77.8 & 81.0 & 72.3 & 75.0 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

Q5) The improvement on Office-Home dataset is incremental. \\
A5) Because of the limitation of VGG-16. We conduct additional experiments on ResNet-50. Due to the limited time, we run the experiments on $6$ randomly selected adaptation settings from Office-Home dataset.
The results show that our method outperforms MME by $1.85\%$.
\begin{table}[h]
    \centering
    \caption{Comparisons of the proposed method and MME on $6$ randomly selected adaptation settings from Office-Home dataset based on VGG-16 and ResNet-50.}
    \label{tab:OfficeHome_withResNet34}
    \begin{tabular}{r|cccccc|c}
        \toprule
        Method & A$\to$C & A$\to$R & C$\to$R & C$\to$P & P$\to$A & P$\to$C & MEAN \\
        \hline
        \multicolumn{8}{c}{Three-shot SSDA on VGG-16} \\
        \hline
        MME & 54.9 & 75.3 & 72.9 & 76.3 & 59.2 & 53.6 & 65.4 \\
        Ours & 55.1 & 76.3 & 73.3 & 76.1 & 59.3 & 53.9 & 65.7 (+0.3) \\
        \hline
        \multicolumn{8}{c}{Three-shot SSDA on ResNet-50 (NEW)} \\
        \hline
        MME & 77.2 & 76.1 & 73.2 & 77.4 & 61.1 & 61.4 & 71.1 \\
        Ours & 78.4 & 77.6 & 76.0 & 79.0 & 64.4 & 63.1 & 73.1 (+2.0) \\
        \bottomrule
    \end{tabular}
\end{table}
%(2) Do you just IGNORE the gains on DomainNet or VisDA-2017?

Q6) The comparison with MME maybe not fair, since the authors introduce additional modules. \\
A6) (i) The goal of this paper is to enhance the discrimination of learned features, rather than a new module that works alone. (ii) Proposing improvements based on existing baselines is one mainstream of how to conduct research, which is no trivial. MME is also based on the entropy and ResNet.


==> figures/fig_OverwhelmingOnSourceDomain.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/PoorDiscriminationOfSOTA.jpg}
    \vspace{-5mm}
    \caption{A t-SNE visualization of the embedded features for the \emph{synthetic-to-real} task from the VisDA-2017 dataset~\cite{peng2017visda}. Features from classes $0$ to $11$ are marked with different colors. (a) Feature distribution in the source domain. Feature distribution in the target domain with (b) ``Drop to Adapt'' (DTA)~\cite{lee2019drop} (a recent UDA method), and (c) Minimax Entropy (MME)~\cite{saito2019semi} (a recent SSDA method).%, and (d) the proposed ELP method.
    This figure is best viewed in the electronic version.
    }
    \label{fig:OverwhelmingOnSourceDomain}
\end{figure}


==> figures/fig_PseudoLabelRefinement.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{images/PseudoLabelRefinement_0.png}
    \caption{The comparisons of different pseudo label refinement methods.}
    \label{fig:PseudoLabelRefinement}
\end{figure}

==> figures/fig_VisualizationOfErrorCurves.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/VisualizationOfErrorCurves.png}
    \caption{The visualizations of error curves on two DA datasets: (a) DomainNet dataset, (b) VisDA-2017 benchmark.}
    \label{fig:VisualizationOfErrorCurves}
\end{figure}

==> sections/3__motivations.tex <==
\begin{itemize}
    % \item "(provide theoretical insight)" from \textit{Manifold Mixup: Better Representations By Interpolating Hidden States}
    
    \item "Previous methods minimize the domain discrepancy neglecting the class information, which may lead to misalignment and poor generalization performance. To address this issue, this paper proposes Contrastive Adaptation Network (CAN) optimizing a new metric which explicitly models the intra-class domain discrepancy and the inter-class domain discrepancy." from \textit{Contrastive Adaptation Network for Unsupervised Domain Adaptation}
    
    \item "However, domain adversarial methods render sub-optimal performances since they attempt to match the distributions among the domains without considering the task at hand." from \textit{Drop to Adapt: Learning Discriminative Features for Unsupervised Domain Adaptation}

    \item "Human adaptability relies crucially on the ability to learn and merge knowledge both from supervised and unsupervised learning: the parents point out few important concepts, but then the children fill in the gaps on their own. This is particularly effective, because supervised learning can never be exhaustive and thus learning autonomously allows to discover invariances and regularities that help to generalize. In this paper we propose to apply a similar approach to the task of object recognition across domains: our model learns the semantic labels in a supervised fashion, and broadens its understanding of the data by learning from self-supervised signals how to solve a jigsaw puzzle on the same images. This secondary task helps the network to learn the concepts of spatial correlation while acting as a regularize for the classification task." from \textit{Domain Generalization by Solving Jigsaw Puzzles}
    \end{itemize}


==> tables/tab_FurtherInvestigationMedian.tex <==
\begin{table}[!t]
    \centering
    \caption{The comparisons of separating the clean data and noisy data by using median and different fixed thresholds. The experiments are conducted on the ``\textit{painting $\to$ clipart}'' of the DomainNet dataset.}
    \label{tab:FurtherInvestigationMedian}
    \footnotesize{
    \begin{tabular}{l|c c c c c}
        \toprule
        Setting & $(0,70\%) $ & $[70\%,90\%)$ & $[90\%,100\%)$ & $100\%$ & SUM\\
        \hline
        Median & 20 & 18 & 59 & 29 & 126 $(87\%)$ \\ 
        \hline
        0.6 & 37 & 49 & 39 & 1 & 126 $(76\%)$ \\
        \hline
        0.7 & 36 & 52 & 37 & 1 & 126 $(78\%)$ \\
        \hline
        0.8 & 33 & 50 & 40 & 3 & 126 $(79\%)$ \\
        \hline
        0.9 & 28 & 42 & 49 & 3 & 126 $(81\%)$ \\
        \bottomrule
    \end{tabular}
    }
\end{table}

